Konzept f\"ur Bildanalysen in Hochdurchsatz-Systemen am Beispiel des Zebrab\"arblings

With image-based high-throughput experiments, new challenges arise in both, the design of experiments and the automated analysis. To be able to handle the massive number of single experiments and the corresponding amount of data, a comprehensive concept for the design of experiments and a new evaluation method is needed. This work proposes a new method for an optimized experiment layout that enables the determination of parameters, adapted for the needs of automated image analysis. Furthermore, a catalogue of new image analysis modules, especially developed for zebrafish analysis, is presented. The combination of both parts offers the user, usually a biologist, an approach for high-throughput zebrafish image analysis, which enables the extraction of new signals and optimizes the design of experiments. The result is a reduction of data amount, redundant information and workload as well as classification errors.

==> Bilder/04_Implementierung_Skalierung/Fremdimplementierungen.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                                                  %%
%%  This is a LaTeX2e table fragment exported from Gnumeric.        %%
%%                                                                  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\href{http://en.wikipedia.org/wiki/CombineZ}{CombineZ}	&Auf die Kombination mehrerer Fokusaufnahmen spezialisierte, batchf\"{a}hige Software	&Alan Hadley	&GPL	\\
\href{http://www.mathworks.de/matlabcentral/fileexchange/26978-hough-transform-for-circles}{Hough transform for circles\footnote{www.mathworks.de/matlabcentral/fileexchange/26978-hough-transform-for-circles}}	&Implementierung des Hough-Algorithmus zur Kreisdetektion	&David Young	&BSD	\\
\href{http://rsb.info.nih.gov/ij/}{ImageJ}	&Bildbearbeitungs- und Bildverarbeitungsprogramm	&Wayne \mbox{Rasband}	&Public Domain	\\
\href{http://www.irfanview.de}{IrfanView}	&Bildbetrachter mit umfangreichen Funktionen	&Irfan \^Skiljan	&Freeware	\\
\href{http://www.ni.com/analysis/lvaddon_vision.htm}{LabVIEW \mbox{add-on:} Vision/Image Processing}	&Bildverarbeitungserweiterung f\"{u}r LabVIEW	&National  \mbox{Instruments}	&Propriet\"{a}r	\\
\href{http://www.mathworks.de/products/image/}{MATLAB Image Processing Toolbox}	&Umfangreiche Sammlung von Bild\-ver\-ar\-bei\-tungs- und Bild\-analyse\-funktionen	&Mathworks	&Propriet\"{a}r	\\
\href{http://www.mathworks.de/matlabcentral/fileexchange/25500-peakfinder}{PeakFinder}\footnote{www.mathworks.de/matlabcentral/fileexchange/25500-peakfinder}	&Implementierung zur Minima- und Maximadetektion innerhalb verrauschter Daten	&Nate Yoder	&BSD	\\
\href{http://de.wikipedia.org/wiki/SyncToy}{Sync-Toy}	&Tool zur Synchronisierung von Dateien und Ordnern	&Microsoft	&Freeware	\\
\href{http://www.mathworks.de/matlabcentral/fileexchange/28590-template-matching-using-correlation-coefficients}{Template Matching using Correlation Coefficients}\footnote{www.mathworks.de/matlabcentral/fileexchange/28590-template-matching-using-correlation-coefficients}	&Implementierung des Template-Matching Verfahrens	&Yue Wu	&BSD	\\
\href{http://de.wikipedia.org/wiki/TortoiseSVN}{TortoiseSVN}	&Windows-Client f\"{u}r den Versions\-ver\-waltungs\--Dienst Subversion-SVN	&The Tortoise\-SVN team	&GPL	\\


==> Bilder/04_Implementierung_Skalierung/Funktionen.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                                                  %%
%%  This is a LaTeX2e table fragment exported from Gnumeric.        %%
%%                                                                  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
calc\_colorbar.m	&Berechnen des Farbcodes f\"{u}r den Plot	&108\\
calc\_movements.m	&Berechnen der Bewegungsreihe	&100\\
CircularHough\_Grd.m	&Hough Kreisdetektion	&664\\
corrMatching.m	&Tracking mittels Korrelation	&79\\
Find\_fish.m	&Segmentierung der Fischeier	&336\\
fish\_gui.m	&Grafische Oberfl\"{a}che von PIMP	&1070\\
fish\_gui\_about.m	&Credits von PIMP	&82\\
fish\_gui\_report\_generator.m	&Grafische Oberfl\"{a}che des Reportgenerators	&352\\
get\_fish\_video.m	&Konvertierung der Bildsequenzen	&35\\
imprctile.m	&Berechnung von Perzentilen zur Normalisierung	&27\\
make\_report.m	&Reportgenerierung	&120\\
MidpointCircle.m	&Erzeugen von Bildern mit Kreisen zum Tracken der Fischeier	&63\\
peakfinder.m	&Auffinden ausgepr\"{a}gter Maxima	&220\\
perfect\_template.m	&Erstellung eines Template zum Tracken	&37\\
show\_fish\_movements.m	&Visualisierung der Bewegungsplots	&112\\
show\_fish\_spectrogram.m	&Visualisierung der Heatmaps	&228\\
show\_fish\_tracking.m	&Visualisierung der getrackten Bildsequenz	&63\\


==> Text/02b_Neues_Konzept_Begriffe.tex <==
Begrifflichkeiten werden in der Literatur zur Versuchsauslegung unterschiedlich verwandt. Um einer Verwechslung vorzubeugen werden wichtige der für diesen Abschnitt notwendigen Begriffe hier kurz definiert. Die Definitionen lehnen sich an die Fachliteratur zur Versuchsplanung an.

Die \hts kann als Grundgesamtheit betrachtet werden, welche die Menge an Objekten ist (\zB hier Modellorganismen oder Zebrabärblingen) über die nach empirischen \emph{Untersuchungen} bestimmter \emph{Merkmale} in einer Teilmenge (Stichprobe) eine Aussage zu treffen ist. Untersuchungen können hierbei sowohl Erhebungen als auch \emph{Versuche} bezeichnen. Der Unterschied liegt darin, dass bei Versuchen eine \emph{aktive Einflussnahme} auf die objektive Realität vorgenommen wird, während bei einer Erhebung lediglich beobachtet wird. Da in dieser Arbeit keine Erhebungen vorkommen wird die Untersuchung häufig auch als Synonym für den Versuch verwendet. Die aktive Einflussnahme wird als \emph{Behandlung} bezeichnet.

Die \emph{Versuchseinheit} bildet die kleinste unterscheidbare Einheit in einem Versuch. Dies ist in den untersuchten Fällen oft der gesamte Zebrabärbling, jedoch kann ein Merkmalsträger (hier der Zebrabärbling) auch mehrere Versuchseinheiten beinhalten, wenn beispielsweise beide Augen, oder mehrere Zellen innerhalb eines Zebrabärblings getrennt betrachtet werden. In diesem Fall wäre das Auge oder die Zelle die kleinste Einheit und bildet somit die Versuchseinheit.

\emph{Merkmale} sind die Versuchseinheiten beobachtende Größen. Es wird zwischen diskreten (Merkmale mit endlichen, \bzw unendlichen Ausprägungen die jedoch nicht abzählbar sind), kontinuierlichen (Merkmale mit überabzählbar vielen Ausprägungen), qualitativen (Merkmale in einer Nominalskala oder Ordinalskala) und quantitativen (Merkmale in Zahlen oder Intervallen) Größen unterschieden \cite{Mikut08}.




==> Text/02d_Neues_Konzept_Strukturierung_Anforderungen_doppelt.tex <==


Nach der Formulierung der Anforderungen in Kapitel \ref{sec:HDU_Anforderungen} und dem Aufzeigen der zur Verf\"{u}gung stehenden Versuchs- und Auswerteparameter besteht eine schwierige Aufgabe darin, die Parameter so auszuw\"{a}hlen, dass die Anforderungen auch erf\"{u}llt werden. Daher wird, um die Struktur der \hts den Anforderungen  entsprechend zu erstellen, im folgenden Kapitel ein Flussdiagramm vorgestellt, welches bei der erfolgreichen Gestaltung eines Hochdurchsatzversuches empfohlen wird. Beim Durchlaufen des Diagramms werden Schritt f\"{u}r Schritt Parameter festgelegt und jeweils gepr\"{u}ft ob die Auslegung den Anforderungen gerecht wird.
\begin{figure}[htbp]
        \centering
        \includegraphics[page=4]{Bilder/Diss_Zusammenhang}
\caption{Flussdiagramm f\"{u}r die anforderungskonforme Strukturierung des Versuchsplans von \htsen}
\label{fig:Ablaufdiagramm_Screendesign}
\end{figure}




In diesem Flussdiagramm werden 4 Versuchspl\"{a}ne erstellt, die zur erfolgreichen Strukturierung erforderlich sind. Versuchsplan f\"{u}r
 \begin{enumerate}
  \item die Identifikation des biologischen Effekts \dhe Ermittlung des Nutzsignals,
  \item die Akquise des Nutzsignals \dhe Durchf\"{u}hrung der Messung,
  \item die Extraktion und Klassifikation der Merkmale \dhe Auswertung des Bildstroms,
  \item die Durchf\"{u}hrung der \hts \dhe die Erstellung des statistischen Versuchsplanes.
\end{enumerate}

Innerhalb der ersten drei Schritte werden nacheinander folgende Bedingungen gepr\"{u}ft, bevor der 4. Punkt, die Durchf\"{u}hrung der \hts, vollzogen werden kann:
\begin{itemize}
  \item Anforderungen an die Durchf\"{u}hrung
  \item Anforderungen an die Messung
  \item Anforderungen an die Auswertung
  \item Skalierbarkeit der \hts
\end{itemize}

Der 1. Schritt, das Finden des biologischen Effekts, ist vollst\"{a}ndig biologisch motiviert. Das \Nutzsig variiert von \hts zu \hts und ist \zB eine anatomische Besonderheit, wie etwa eine gelabelte Zelle. Andere Beispiele sind ein besonderer Ph\"{a}notyp, eine Reaktion auf einen Stimulus, ein Bewegungsmuster \usw Entscheidend f\"{u}r die technische Durchf\"{u}hrbarkeit der \hts ist, ob der biologische Effekt reproduziert werden kann. Dieser Schritt kann durch einfaches Wiederholen des biologischen Versuchs gepr\"{u}ft werden. Ist dies nicht gegeben, so ist mit diesem Effekt keine \hts m\"{o}glich und ein anderer, besser geeigneter Effekt muss gew\"{a}hlt werden. Der Schritt vereint die beiden Arbeitsschritte  "`Versuchsplanung"' und "`Vorbereitung"' in \abb \ref{fig:Assay_Gestaltung}.

Wurde ein reproduzierbarer biologischer Effekt gefunden wird versucht, das \Nutzsig zu akquirieren. Die Akquise ist f\"{u}r alle existierenden Akquise-Methoden gleichbedeutend mit einer r\"{a}umlichen und einer zeitlichen Abtastung sowie einer Quantisierung. Die gew\"{a}hlte Methode muss dabei:
 \begin{itemize}
   \item Die Zebrab\"{a}rblingslarve und insbesondere das \Nutzsig robust abbilden.
   \item Ein gutes \Nutzsig-Rausch-Verh\"{a}ltnis aufweisen.
   \item Dem Abtasttheorem approximativ gerecht werden.
 \end{itemize}
Dies kann in den Bildern meist durch einfaches Ansehen der Bilder gepr\"{u}ft werden. Sind die auszuwertenden Bereiche beispielsweise ein Gewebe in der Larve, so ist auf einen guten Kontrast dieser Bereiche zu achten. Beim \"{U}berpr\"{u}fen der gew\"{a}hlten Abtastfrequenz und bei mit niedriger Frequenz auftretenden \Nutzsigen muss deren Frequenz zuvor mittels entsprechenden Messeinrichtungen ermittelt werden. Eine m\"{o}glichst vollst\"{a}ndige Repr\"{a}sentation des \Nutzsigs im akquirierten Bildstrom muss angestrebt werden. Die gro{\ss}e Bandbreite an m\"{o}glichen biologischen Effekten und damit \Nutzsigen  l\"{a}sst eine allgemein g\"{u}ltige Empfehlung nicht zu. Die Erfahrung zeigt jedoch, dass sich Daten qualitativ f\"{u}r eine automatische Auswertung eignen, wenn es einem unge\"{u}bten menschlichen Betrachte m\"{o}glich ist das \Nutzsig im Bildstrom leicht zu identifizieren und \ggf zu markieren. Andernfalls muss eine alternative Methode zur Bildakquise angewandt werden oder der biologische Effekt muss verworfen werden. Die Akquise ist in \abb \ref{fig:Assay_Gestaltung} durch den Block "`Mikroskopie"'. Das Ergebnis der Akquise ist der Bildstrom.

Ist das \Nutzsig robust im Bildstrom enthalten, besteht der dritte Schritt darin, Methoden der Bildverarbeitung anzuwenden, um dieses aus dem Bildstrom zu extrahieren und daraufhin ein oder mehrere Merkmale zu extrahieren, die das \Nutzsig und dessen Ver\"{a}nderung in Zahlenwerten wiedergeben. Die Segmentierung fasst inhaltlich zusammengeh\"{o}rige Regionen zusammen und wird bei der \hts angewandt, um die \NutzsigInf vom \"{u}brigen Bildstrom zu trennen. Ziel der Segmentierung ist es, die zusammengeh\"{o}renden Regionen des \Nutzsigs (die \NutzsigInf) vom Hintergrund zu unterscheiden. Als Hintergrund werden all diejenigen Bereiche betrachtet, welche nicht zum \Nutzsig geh\"{o}ren. F\"{u}r die Segmentierung l\"{a}sst sich im Bezug auf die \hts als Forderung formulieren:
\begin{itemize}
    \item Das \Nutzsig muss durch die Segmentierung von anderen Informationen  im Datensatz getrennt werden.
  \item Die Segmentierung muss m\"{o}glichst robust sein. Toleranzen in Helligkeit, Reflexionen, Lage des Objekts \ua m\"{u}ssen m\"{o}glichst abgefangen sein.
  \item Der Berechnungsaufwand soll m\"{o}glichst gering sein.

\end{itemize}
Der dritte Schritt in \abb \ref{fig:Ablaufdiagramm_Screendesign} ist die Extraktion von Merkmalen aus dem Bildstrom. Ein Merkmal bezeichnet eine aus akquirierten Daten abgeleitete Gr\"{o}{\ss}e. Merkmale m\"{u}ssen zwar, je nach \Nutzsig der \hts, unterschiedlichen Bedingungen gerecht werden, dennoch lassen sich allgemein g\"{u}ltige Forderungen formulieren:
\begin{enumerate}
  \item Vom \Nutzsig unabh\"{a}ngige Gr\"{o}{\ss}en (wie etwa die Beleuchtung) d\"{u}rfen die Merkmale nicht oder nur unwesentlich beeinflussen.
  \item Der Berechnungsaufwand soll m\"{o}glichst gering sein.
  \item Die univariate Trenng\"{u}te muss gew\"{a}hrleistet sein. \Dh jedes Merkmal muss f\"{u}r sich in der Lage sein, die betrachteten Klassen des \Nutzsigs zu trennen.
  \item Die multivariante Trenng\"{u}te muss gew\"{a}hrleistet sein. \Dh die Kombination der Merkmale muss eine gute Unterscheidung der Klassen des \Nutzsigs erlauben.
  \item Die Auspr\"{a}gungen der Merkmale m\"{u}ssen m\"{o}glichst robust sein und daher eine geringe Empfindlichkeit gegen\"{u}ber Signalrauschen, Messfehlern oder zeitvarianten \"{A}nderungen aufweisen.

\end{enumerate}
K\"{o}nnen keine oder nur unzureichend beschreibende Merkmale gefunden werden, muss gepr\"{u}ft werden, ob mittels einer anderen Akquise-Methode aussagekr\"{a}ftige Merkmale extrahiert werden k\"{o}nnen. Ist dies nicht der Fall, muss der biologische Effekt verworfen werden.

Nach erfolgreicher Merkmalsextraktion ist das \Nutzsig durch Zahlenwerte abgebildet und es muss abschlie{\ss}end gepr\"{u}ft werden, ob der Umfang der \hts mit der ausgearbeiteten L\"{o}sung durchgef\"{u}hrt werden kann. Auf der Basis der bis zu diesem Zeitpunkt verf\"{u}gbaren Informationen kann eine Hochrechnung f\"{u}r die wichtigsten Anforderungen f\"{u}r den Versuch erfolgen. Zu ber\"{u}cksichtigende Werte sind
die Akquisezeit, der notwendige Speicherplatz, die notwendige Rechenkapazit\"{a}t und zur Verf\"{u}gung stehende Computer Hardware, die zur Verf\"{u}gung stehenden iModellorganismen, der Durchsatz der Mikroskopplattformen sowie die Arbeitskraft f\"{u}r die manuell durchzuf\"{u}hrenden Schritte. Die berechneten Anforderungen m\"{u}ssen mit den zur Verf\"{u}gung stehenden Mitteln verglichen werden. Ist die Untersuchung nicht durchf\"{u}hrbar, m\"{u}ssen Parameter skaliert werden. Eine M\"{o}glichkeit bietet \zB das Anpassen der Anzahl von Einzelexperimenten. Bez\"{u}glich des Modellorganismuses kann auf einen gr\"{o}{\ss}eren oder kleineren Organismus ausgewichen werden. Beim Zebrab\"{a}rbling l\"{a}sst sich \zB die Gr\"{o}{\ss}e durch das Alter skalieren, \dhe durch das Verwenden j\"{u}ngerer oder \"{a}lterer Fische \bzw Larven. Auch die Anzahl gleichzeitig akquirierter Modellorganismen kann variiert werden. Ebenso ist das Verwenden von mehreren Mikroskopen zur Erh\"{o}hung des Durchsatzes m\"{o}glich.

Der angesprochene Vorteil der Skalierbarkeit der Versuche durch die Vorteile des Zebrab\"{a}rblings ist jedoch auch mit Nachteilen verbunden. Die kleine Gr\"{o}{\ss}e der Larven und die hohe Legerate der Elterntiere erm\"{o}glicht zwar das einfache Bereitstellen einer hohen Anzahl an Modellorganismen, jedoch ist das \Nutzsig bei sehr jungen Tieren oft abgeschw\"{a}cht gegen\"{u}ber dem der ausgewachsenen Tiere. Werden mehrere Larven gleichzeitig akquiriert, erh\"{o}ht dies zwar den Durchsatz, die Larven k\"{o}nnen sich jedoch gegenseitig beeinflussen und damit das \Nutzsig st\"{o}ren. Diese m\"{o}glichen St\"{o}rungen  m\"{u}ssen f\"{u}r eine sp\"{a}tere Auswertung ber\"{u}cksichtigt werden oder \ggf beseitigt werden. Ein weiterer Aspekt ist, dass der Aufwand f\"{u}r die Bildverarbeitung steigt, wenn die Versuchseinheit das Einzelindividuum ist, jedoch mehrere Versuchseinheiten gleichzeitig akquiriert werden. In diesem Fall m\"{u}ssen die Larven im Bild durch die Bildverarbeitung getrennt werden. Bei Bildsequenzen ist in diesen F\"{a}llen zus\"{a}tzlich ein Tracking und m\"{o}glicherweise eine Regression der separierten Versuchseinheiten notwendig.

Wichtig bei der Skalierung ist, dass sich bei Anwendung einer der aufgezeigten L\"{o}sungsvorschl\"{a}ge (oder auch anderer) diese Ver\"{a}nderung auf jeden Schritt der Untersuchung auswirkt, wie im Konzept in Kapitel \ref{sec:Konzept_Versuchsauslegung} erarbeitet. Daher muss nach jeder Iteration das \emph{gesamte} Flussdiagramm nochmals durchlaufen werden. Erst wenn die \hts in der gew\"{u}nschten Weise ohne weitere Anpassungen durchf\"{u}hrbar ist, darf mit der tats\"{a}chlichen Ausf\"{u}hrung des Experiments begonnen werden. Ein typischer Fehler ist es, w\"{a}hrend der Durchf\"{u}hrung den Prozess durch skalierende Ma{\ss}nahmen zu beschleunigen. Dies f\"{u}hrt oftmals zu St\"{o}rfaktoren, deren Einfluss sich nicht beseitigen l\"{a}sst oder gar zum Scheitern der \hts f\"{u}hrt.



==> Text/_00_Zusammenfassung_Bildchen.tex <==
\pagestyle{empty}
%\addtolength{\topmargin}{.875in}
%\addtolength{\leftmargin}{-5in}
%\addtolength{\oddsidemargin}{-1in}
%\addtolength{\evensidemargin}{-.875in}

\begin{centering}
   \includegraphics[page=1,width=\linewidth]{Bilder/Diss_Zusammenhang}
   \vspace{.3cm}
   \includegraphics[page=2,width=\linewidth]{Bilder/Diss_Zusammenhang}
   \vspace{.3cm}
   \includegraphics[page=3,width=\linewidth]{Bilder/Diss_Zusammenhang}
   \vspace{.3cm}
    \includegraphics[page=6,width=\linewidth]{Bilder/Diss_Zusammenhang}
  \begin{landscape}
     \includegraphics[page=4,width=.45\linewidth]{Bilder/Diss_Zusammenhang}
   \includegraphics[page=7,width=.45\linewidth]{Bilder/Diss_Zusammenhang}\\
  \begin{minipage}[b]{0.35\linewidth}
   \includegraphics[page=5,width=\linewidth]{Bilder/Diss_Zusammenhang}
   \end{minipage}
   \begin{minipage}[b]{0.5\linewidth}
   \includegraphics[page=2,width=\linewidth]{Bilder/Diss_Zusammenhang}\\
   \vspace{2cm}\\
   \includegraphics[page=9,width=\linewidth]{Bilder/Diss_Zusammenhang}
   \end{minipage}
     \end{landscape}
    \end{centering}


